Modeling alpha particle-induced radioluminescence using GEANT4

Optical detection of alpha particle emitters in the environment by air radioluminescence is a new technology that enables sensing a radiological threat at safe distances, without putting personnel at risk or contaminating equipment. Radioluminescence detection systems need to be fine-tuned to efficiently capture a substantial number of photons while minimizing the contribution from ambient ultraviolet light. The accurate simulation of radioluminescence, in conjunction with ray tracing, facilitates the design and optimization of such detection systems. In this work, an application within the Geant4 framework has been developed to simulate radioluminescence photons emitted in the vicinity of accelerated alpha particles and at the surface of alpha radioactive samples. The application relies on existing scintillation physics implemented in Geant4 classes such as G4OpticalPhysics and G4Scintillation, which are used to simulate radioluminescence photons as scintillations produced during the passage of alpha particles through air. The application computes the ultraviolet image of alpha particles accelerated at energies of 5.1 MeV and 8.3 MeV, as well as an extended alpha source. The application enables optimization of experimental setups for various scenarios, such as radiological emergency management, radiological crime scene investigations, or decommissioning of nuclear facilities, thus minimizing the use of costly resources and exposure to radiation.

==> rjp_mathdefs.tex <==
%This file contains a hopefully ever growing collection of command shortcuts and even new LaTeX commands (especially for math mode),
%that are currently in use and accepted by Romanian Journal of Physics.
% Last modified: 16/09/2016 (dd/mm/yyyy)
%
% Commands specifically designed for class documentation
\ifrjpcl@ssdoc
\newcommand{\miktex}{\hbox{Mik\kern-.15em\TeX}}
\newcommand{\earXiv}{\texttt{ar\raisebox{-.25ex}{X}iv}}
\newcommand{\texlive}{\hbox{\TeX Live}}
\newcommand{\texcom}[1]{\texttt{\small\textbackslash #1}}
%\newcommand{\rjpurl}[1]{\href{#1}{\texttt{\small #1}}}
\fi
% Environment and general command shortcuts
\providecommand{\beq}[1][\@empty]{\def\@ttoken{#1}\begin{equation}\dbg@ut{\@ttoken}\ifx\@empty#1 \else\label{#1}\fi}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqn}{\begin{equation*}}
\newcommand{\eeqn}{\end{equation*}}
%
% Various other operators
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Img}{Im}
\DeclareMathOperator{\Rel}{Re}
\DeclareMathOperator{\ee}{e}
%
% Elliptic Jacobi functions - obsolete, do not use! (see below)
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\cn}{cn}
\DeclareMathOperator{\dn}{dn}
%
% Mathematical operators and various symbols
\DeclareMathOperator{\ddiv}{div}
\DeclareMathOperator{\grad}{grad}
% Replaceable by \tanh^{-1}
% Hyperbolic functions
\DeclareMathOperator{\artanh}{artanh}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\cosech}{csch}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\cosec}{cosec}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\cc}{\ifmmode\mathrm{cc.\;}\else\textrm{cc.~}\fi}
\newcommand{\ict}{\ifmmode\mathcal{C}\else\texttt{C}\fi}
% Partial derivative
\providecommand{\pd}{\ensuremath{\partial}}
% To be eliminated in future versions!
\providecommand{\dd}{\ensuremath{\mathrm{d}}}
\providecommand{\id}{\ensuremath{\;\mathrm{d}}}
% Full derivative
\providecommand{\fd}{\ensuremath{\mathrm{d}}}
% Bras and Kets
\providecommand{\bra}[1]{\ensuremath{\left<#1\right|}}
\providecommand{\ket}[1]{\ensuremath{\left|#1\right>}}
% the \braket command is thought to be the matrix element of operator #1 for state #2 (left) and state #3 (right)
\providecommand{\braket}[3]{\ensuremath{\left<#2|#1|#3\right>}}
%
% Commands for multiple indexes around a central token #1
% The names derive from "front up-down, back up-down" of #1 (it better be read as "left up-down, right up-down") indicating 
% the order in which indexes are passed starting with #2 (left-up or front-up). The only cool stuff about these commands is 
% that it reduces the space between up-down left indexes and the following token.
\newcommand{\fudbud}[5]{{\!\;}^{#2}_{#3}\!\!#1^{#4}_{#5}}
\newcommand{\fubu}[3]{{\!\;}^{#2}\!\!#1^{#3}}
\newcommand{\fdbd}[3]{{\!\;}_{#2}\!\!#1_{#3}}
\newcommand{\fdbu}[3]{{\!\;}_{#2}\!#1^{#3}}
\newcommand{\fubd}[3]{{\!\;}^{#2}\!#1_{#3}}
%
% put a small hat on operators!
\providecommand{\hatop}[1]{\ensuremath{\hat{\mathop{\operator@font #1}\nolimits}}}
%
% A small macro for generating uppercased letters of specific math font (mathfrak).
\let\op@format\mathfrak
% \let\op@format\mathcal
\def\op#1{%
 \ifnum`#1=\lccode`#1
  \expandafter\ensuremath\op@format{\uppercase{#1}}
 \else%
  \expandafter\ensuremath\op@format{#1}
 \fi%
}%
% Jacobi elliptic functions as operators
\DeclareMathOperator{\jsn}{sn} % to replace duplicates above!
\DeclareMathOperator{\jcn}{cn}
\DeclareMathOperator{\jdn}{dn}
\DeclareMathOperator{\jns}{ns} % 1/sn(u)
\DeclareMathOperator{\jnc}{nc} % 1/cn(u)
\DeclareMathOperator{\jnd}{nd} % 1/dn(u)
\DeclareMathOperator{\jsc}{sc} % sn(u)/cn(u)
\DeclareMathOperator{\jsd}{sd} % sn(u)/dn(u)
\DeclareMathOperator{\jdc}{dc} % dn(u)/cn(u)
\DeclareMathOperator{\jds}{ds} % dn(u)/sn(u)
\DeclareMathOperator{\jcs}{cs} % cn(u)/sn(u) 
\DeclareMathOperator{\jcd}{cd} % cn(u)/dn(u)

% Pre-formatted special text chunks
\providecommand{\ie}{\textit{i.e.}}
\providecommand{\eg}{\textit{e.g.}}
\providecommand{\etal}{\textit{et al.}}



